A JWST/MIRI and NIRCam Analysis of the Young Stellar Object Population in the Spitzer I region of NGC 6822

We present an imaging survey of the Spitzer I star-forming region in NGC 6822 conducted with the NIRCam and MIRI instruments onboard JWST. Located at a distance of 490 kpc, NGC 6822 is the nearest non-interacting low-metallicity ($\sim$0.2 $Z_{\odot}$) dwarf galaxy. It hosts some of the brightest known HII regions in the local universe, including recently discovered sites of highly-embedded active star formation. Of these, Spitzer I is the youngest and most active, and houses 90 color-selected candidate young stellar objects (YSOs) identified from Spitzer Space Telescope observations. We revisit the YSO population of Spitzer I with these new JWST observations. By analyzing color-magnitude diagrams (CMDs) constructed with NIRCam and MIRI data, we establish color selection criteria and construct spectral energy distributions (SEDs) to identify candidate YSOs and characterize the full population of young stars, from the most embedded phase to the more evolved stages. In this way, we have identified 140 YSOs in Spitzer I. Comparing to previous Spitzer studies of the NGC 6822 YSO population, we find that the YSOs we identify are fainter and less massive, indicating that the improved resolution of JWST allows us to resolve previously blended sources into multiple objects.

==> Tables/color_cuts_v1.tex <==
\begin{deluxetable*}{lc}
\label{tab:color_cuts}
\tabletypesize{\normalsize}
\tablewidth{0pt}
\tablecaption{
Color Selection Criteria Used to Identify Red Sources
}
\tablehead{\colhead{Color Selection}&\colhead{Number of Sources} \\
}
\startdata
F770W$-$F1500W $\geq 0.6$ and $14 \leq \mathrm{F1500W} \leq 18$ & 38 \\
F1000W$-$F1500W $\geq 0.6$ and $14 \leq \mathrm{F1500W} \leq 18$ & 29 \\
F356W$-$F770W $\geq 0.6$ and $15.5 \leq \mathrm{F770W} \leq 19.8$ & 154 \\
F444W$-$F770W $\geq 0.6$ and $15.5 \leq \mathrm{F770W} \leq 19.8$ & 145 \\
$\mathrm{y} > -8.9\,\mathrm{x} + 33.7$ and $\mathrm{y} > -0.2\,\mathrm{x} + 18.0$ and $\mathrm{y} < -0.2\,\mathrm{x} + 23.5$ & 780$^{a}$ \\
$\mathrm{y} > -9.7\,\mathrm{x} + 34.9$ and $\mathrm{y} > -0.2\,\mathrm{x} + 17.7$ and $\mathrm{y} < -0.2\,\mathrm{x} + 23.6$ & 750$^{b}$ \\
\enddata
\tablecomments{$^{a}$Here y corresponds to the F444W magnitude, and x corresponds to the F115W$-$F444W color. $^{b}$Here y corresponds to the F356W magnitude, and x corresponds to the F115W$-$F356W color.}
\end{deluxetable*}


==> Tables/observations.tex <==
\begin{deluxetable*}{ccccccc}
\label{tab:obs_params}
\tabletypesize{\normalsize}
\tablewidth{0pt}
\tablecaption{
Observing Parameters for NIRCam MIRI Prime Imaging
}
\tablehead{
\colhead{Filter}&\colhead{Field}&\colhead{Readout Pattern}&\colhead{Groups/Int.}&\colhead{Int./Exp.}&\colhead{Dithers}&\colhead{Total Exp.\ Time}
\\
& & & & & & [sec]
}
\startdata
\cutinhead{NIRCam}
F115W & NIRCam Prime & \textsc{bright2} & 7 & 1 & 12 & 1803.777 \\
F200W & NIRCam Prime & \textsc{bright2} & 7 & 1 & 12 & 1803.777 \\
F356W & NIRCam Prime & \textsc{bright2} & 7 & 1 & 12 & 1803.777 \\
F444W & NIRCam Prime & \textsc{bright2} & 7 & 1 & 12 & 1803.777 \\
\cutinhead{MIRI}
F770W & MIRI Prime & \textsc{fastr1} & 52 & 1 & 4 & 577.208 \\
F1000W & MIRI Prime & \textsc{fastr1} & 36 & 2 & 4 & 810.312 \\
F1500W & MIRI Prime & \textsc{fastr1} & 15 & 8 & 4 & 1409.72 \\
F2100W & MIRI Prime & \textsc{fastr1} & 20 & 9 & 4 & 2086.83 \\
\enddata
\tablecomments{Comments here.}
\end{deluxetable*}

% \begin{deluxetable*}{ccccccc}
% \label{tab:obs_params_NIRCam}
% \tabletypesize{\small}
% \tablewidth{0pt}
% \tablecaption{
% Observing Parameters for NIRCam Imaging
% }
% \tablehead{
% \colhead{Filter}&\colhead{Field}&\colhead{Readout Pattern}&\colhead{Groups/Int.}&\colhead{Int./Exp.}&\colhead{Dithers}&\colhead{Total Exp.\ Time}
% \\
% & & & & & & [sec]
% }
% \startdata
% F115W & NIRCam Prime & \textsc{bright2} & 7 & 1 & 12 & 1803.777 \\
% F200W & NIRCam Prime & \textsc{bright2} & 7 & 1 & 12 & 1803.777 \\
% F356W & NIRCam Prime & \textsc{bright2} & 7 & 1 & 12 & 1803.777 \\
% F444W & NIRCam Prime & \textsc{bright2} & 7 & 1 & 12 & 1803.777 \\
% \hline
% F140M & NIRCam Parallel (MIRI) & \textsc{shallow4} & 8 & 1 & 4 & 1674.936 \\
% F335M & NIRCam Parallel (MIRI) & \textsc{shallow4} & 8 & 1 & 4 & 1674.936 \\
% F115W & NIRCam Parallel (MIRI) & \textsc{shallow2} & 3 & 1 & 4 & 515.365 \\
% F150W & NIRCam Parallel (MIRI) & \textsc{shallow2} & 4 & 1 & 4 & 730.100 \\
% F200W & NIRCam Parallel (MIRI) & \textsc{shallow4} & 4 & 1 & 4 & 815.995 \\
% F277W & NIRCam Parallel (MIRI) & \textsc{shallow2} & 4 & 1 & 4 & 730.100 \\
% F356W & NIRCam Parallel (MIRI) & \textsc{shallow2} & 3 & 1 & 4 & 515.365 \\
% F444W & NIRCam Parallel (MIRI) & \textsc{shallow4} & 4 & 1 & 4 & 815.995 \\
% \enddata
% \tablecomments{Comments here.}
% \end{deluxetable*}

% \begin{deluxetable*}{ccccccc}
% \label{tab:obs_params_MIRI}
% \tabletypesize{\small}
% \tablewidth{0pt}
% \tablecaption{
% Observing Parameters for MIRI Imaging
% }
% \tablehead{
% \colhead{Filter}&\colhead{Field}&\colhead{Readout Pattern}&\colhead{Groups/Int.}&\colhead{Int./Exp.}&\colhead{Dithers}&\colhead{Total Exp.\ Time}
% \\
% & & & & &  & [sec]
% }
% \startdata
% F770W & MIRI Prime & \textsc{fastr1} & 52 & 1 & 4 & 577.208 \\
% F1000W & MIRI Prime & \textsc{fastr1} & 36 & 2 & 4 & 810.312 \\
% F1500W & MIRI Prime & \textsc{fastr1} & 15 & 8 & 4 & 1409.72 \\
% F2100W & MIRI Prime & \textsc{fastr1} & 20 & 9 & 4 & 2086.83 \\
% \hline
% F1000W & MIRI Parallel (NIRCam) & \textsc{slowr1} & 5 & 1 & 12 & 1433.395 \\
% F1500W & MIRI Parallel (NIRCam) & \textsc{slowr1} & 5 & 1 & 12 & 1433.395 \\
% \enddata
% \tablecomments{Comments here.}
% \end{deluxetable*}

==> Tables/properties_v1.tex <==
\begin{deluxetable*}{lcccccc}
\label{tab:props}
\tabletypesize{\normalsize}
\tablewidth{0pt}
\tablecaption{Physical properties of \emph{JWST}-Identified YSOs in Spitzer~I }
\tablehead{
    \colhead{Source}        &
    \colhead{RA}            &
    \colhead{Dec.}           &
    \colhead{Radius, $R_{*}$}       &
    \colhead{Temperature, $T_{\mathrm{eff}}$} &
    \colhead{Luminosity, $L_{*}$}       &
    \colhead{Mass, $M_{*}$}       \\
    \colhead{}              &
    \colhead{(J2000)}       &
    \colhead{(J2000)}        &
    \colhead{[R$_{\odot}$]} &
    \colhead{[K]}           &
    \colhead{[L$_{\odot}$]} &
    \colhead{[M$_{\odot}$]}\\
}
\startdata
1 & 296.2357315 & -14.80020774 & 9.38 & 7219 & 216 & 4.64\\
4 & 296.2380947 & -14.79751884 & 33.01 & 8087 & 4208 & 10.85\\
5 & 296.2417682 & -14.80489326 & 73.23 & 3381 & 633 & 6.31 \\
6 & 296.2450078 & -14.80011861 & 99.46 & 3108 & 833 & 6.83 \\
7 & 296.2528028 & -14.80153774 & 49.17 & 2743 & 124 & 3.96 \\
8 & 296.2518381 & -14.80104333 & 9.74 & 7056 & 212 & 4.62 \\
9 & 296.2514835 & -14.79551891 & 7.55 & 7861 & 196 & 4.52 \\
10 & 296.2376577 & -14.79443789 & 82.56 & 2126 & 126 & 3.98 \\
12 & 296.2397253 & -14.78726164 & 21.76 & 6287 & 668 & 6.41 \\
13 & 296.2398122 & -14.79551639 & 49.58 & 4562 & 961 & 7.12 \\
14 & 296.2429828 & -14.78714408 & 20.46 & 13650 & 13120 & 15.02 \\
15 & 296.2492044 & -14.78996949 & 47.36 & 5125 & 1397 & 7.92 \\
16 & 296.2514153 & -14.79192801 & 78.23 & 4338 & 1957 & 8.72 \\
17 & 296.2506962 & -14.79673471 & 31.68 & 3596 & 151 & 4.20 
\enddata
\tablecomments{The 14 sources listed here correspond to the sources shown in Figure \ref{fig:seds}. The full table is available online.}
\end{deluxetable*}
